Positive and negative mass solitons in spin-orbit coupled Bose-Einstein condensates

We present a unified description of different types of matter-wave solitons that can emerge in quasi one-dimensional spin-orbit coupled (SOC) Bose-Einstein condensates (BECs). This description relies on the reduction of the original two-component Gross-Pitaevskii SOC-BEC model to a single nonlinear Schr\"{o}dinger equation, via a multiscale expansion method. This way, we find approximate bright and dark soliton solutions, for attractive and repulsive interatomic interactions respectively, for different regimes of the SOC interactions. Beyond this, our approach also reveals "negative mass" regimes, where corresponding "negative mass" bright or dark solitons can exist for repulsive or attractive interactions, respectively. Such a unique opportunity stems from the structure of the excitation spectrum of the SOC-BEC. Numerical results are found to be in excellent agreement with our analytical predictions.

==> rrp_mathdefs.tex <==
%\newcommand{\opL}{\mathfrak{L}}
%\newcommand{\opN}{\mathfrak{N}}

%elliptic Jacobi functions
\DeclareMathOperator{\sn}{sn}
\DeclareMathOperator{\cn}{cn}
\DeclareMathOperator{\dn}{dn}

\newcommand{\ddiv}{\ensuremath{\mathop{\operator@font div}\nolimits}}
\newcommand{\grad}{\ensuremath{\mathop{\operator@font grad}\nolimits}}
\newcommand{\artanh}{\ensuremath{\mathop{\operator@font artanh}\nolimits}}
\newcommand{\sech}{\ensuremath{\mathop{\operator@font sech}\nolimits}}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\cc}{\ifmmode\mathrm{cc.\;}\else\textrm{cc.~}\fi}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\ict}{\ifmmode\mathcal{C}\else\texttt{C}\fi}

\let\op@format\mathfrak
%\let\op@format\mathcal
\def\op#1{%
 \ifnum`#1=\lccode`#1
  \expandafter\ensuremath\op@format{\uppercase{#1}}
 \else%
  \expandafter\ensuremath\op@format{#1}
 \fi%
}%

